Toward Unsupervised Outlier Model Selection

Today there exists no shortage of outlier detection algorithms in the literature, yet the complementary and critical problem of unsupervised outlier model selection (UOMS) is vastly understudied. In this work we propose ELECT, a new approach to select an effective candidate model, i.e. an outlier detection algorithm and its hyperparameter(s), to employ on a new dataset without any labels. At its core, ELECT is based on meta-learning; transferring prior knowledge (e.g. model performance) on historical datasets that are similar to the new one to facilitate UOMS. Uniquely, it employs a dataset similarity measure that is performance-based, which is more direct and goal-driven than other measures used in the past. ELECT adaptively searches for similar historical datasets, as such, it can serve an output on-demand, being able to accommodate varying time budgets. Extensive experiments show that ELECT significantly outperforms a wide range of basic UOMS baselines, including no model selection (always using the same popular model such as iForest) as well as more recent selection strategies based on meta-features.

==> algo1.tex <==

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\renewcommand{\algorithmiccomment}[1]{\hfill$\blacktriangleright$ #1}
\newcommand{\cdash}{\multicolumn{1}{c}{--} }


% \newcommand{\super}{$^\blacktriangle$}


% \newcommand{\qap}{$\bm{q}_{\textbf{AP}}$}
% \newcommand{\qroc}{$\bm{q}_{\textbf{ROC}}$}
% \newcommand{\qprn}{$\bm{q}_{\textbf{Prec}}$}

% \newcommand{\Prob}{\mathbb{P}}

% \newcommand{\mE}{\mathcal{E}}
% \newcommand{\mS}{\mathcal{S}}
% \newcommand{\mD}{\mathcal{D}}
% \newcommand{\mV}{\mathcal{V}}
% \newcommand{\mL}{\mathcal{L}}
% \newcommand{\mW}{\mathcal{W}}

% \vspace{-0.2in}
\begin{algorithm}[!ht]
	\caption{\method: Offline and Online Phases}
	\label{algo:metaod_plus}
	\small{
	\begin{algorithmic}[1]
		\REQUIRE (Offline) meta-train database $\mDt = \{(\bX_i, \by_i)\}_{i=1}^n$, model set $\mM$; (Online) new OD dataset $\mD_{\text{test}}=(\bXs, \emptyset)$ (no labels), the neighbor set size $t$, patience $p$, time budget $b$ (optional)
		\ENSURE (Offline) UOMS meta-learner; (Online) Selected model for $\mD_{\text{test}}$
		\algrule
% 		\STATE Train and evaluate $\mM$ on $\mDt$ to get outlier score matrix $\bO$ and performance matrix $\bP$
		\textcolor{blue}{$\blacktriangleright$ (Offline) \textbf{Meta-train}: \textit{Learn predictive function of %to quantify
		task similarity}} {{\textcolor{blue}{\ttfamily{\bf (\S \ref{sec:method})}}}}
		


		\STATE Train each $M_j \in \mM$ on each $\bX_i$ of $\mD_i \in \mDt$ to get outlier scores $\mO_{i,j}$,  $\forall\; i=1\ldots n, \; j=1\ldots m$. 

		\STATE Evaluate each $\mO_{i,j}$ against ground-truth labels $\by_i$ to get performance matrix $\bP \in \R^{n\times m}$, where 
		$\bP_{i,j} := \text{perf}(\mO_{i,j} | \by_i)$
		
		\STATE Define task similarity by weighted Kendall's tau ($\tau$) \COMMENT{\S\ref{subsec:sim}}
% 		(\S\ref{subsubsec:weighted_kendall})


		\STATE Compute Internal Perf. Measures, $\bmij := \phi(\mO_{i,j})$ \COMMENT{\S
		\ref{ssec:ipm}
		%\ref{subsubsec:internal_measure}
		}
		\STATE Train regressor $f(\cdot)$ to predict performance gap $(\bP_{i,j}-\bP_{i,j'})$ from respective IPMs $\bmij$ and $\bmijp$
% 		\la{connection to $\tau$ missing? what is this learning?}
% 		difference 
		\COMMENT{\S
		\ref{ssec:performance_predictor}
		%\ref{subsubsec:regressor}
		}
		\STATE \textbf{Save}  measure $\tau$,  IPM extractor $\phi$, and  regressor $f$ 
		
		
		\algrule
		\textcolor{blue}{$\blacktriangleright$ (Online) \textbf{Model Selection}: \textit{Adaptively identify the similar historical tasks and output the best model}} {{\textcolor{blue}{\ttfamily{\bf (\S \ref{sec:online_model_selection})}}}}
		\STATE Initialize model subset $\mM_s$
% 		, the candidate set $\mM_c := \mM \setminus \mM_s$ 
		 \COMMENT{\S\ref{sssec:init}}
		\REPEAT
		\STATE  Update the neighbor set $\mN$ 
		based on $\mM_s$ 
		\COMMENT{\S\ref{ssec:neighbors}} 
			\STATE  Acquire the model $M^*$ based on $\mN$ that provides the best explore-exploit trade-off, update $\mM_s:= \mM_s \cup M^*$ %\COMMENT
			\hspace{0.675in}
			$\blacktriangleright$ {\S \ref{subsubsec:adptive_search}}
			%model subset $\mM_s:= \mM_s \cup M^*$ based on $\mN$, where  \quad\quad  $M^*$ provides the best explore-exploit trade-off   
			
		%\STATE Check convergence and decrement time budget \COMMENT{\S \ref{?}}
		%\ENDWHILE
		 \UNTIL{not converged w.r.t $p$ \& budget $b$ not exhausted
		\COMMENT{\S \ref{subsubsec:convergence}}
		}
         \STATE {\bf Select} for $\mDs$ the model with maximum avg. performance over $\mN$:   
        $\argmax_{M_j \in \mM} \frac{1}{|\mN|}\sum_{\mD_i \in \mN} \bP_{i, j}$ \quad
       % \COMMENT{Eq. (\ref{equ:selected_model})}
	\end{algorithmic}
	}
\end{algorithm}
\setlength{\textfloatsep}{0.0in}
\vspace{-0.1in}
% \pagebreak



==> submitted_abstract.tex <==
Today there exists no shortage of outlier detection algorithms in the literature, yet the complementary and critical problem of unsupervised outlier model selection (UOMS) is vastly understudied. In this work we propose ELECT, a new approach to select an effective candidate model, i.e. an outlier detection algorithm and its hyperparameter(s), to employ on a new dataset without any labels. At its core, ELECT is based on meta-learning; transferring prior knowledge (e.g. model performance) on historical datasets that are similar to the new one to facilitate UOMS. Uniquely, it employs a dataset similarity measure that is performance-based, which is more direct and goal-driven than other measures used in the past. ELECT adaptively searches for similar historical datasets, as such, it can serve an output on-demand, being able to accommodate varying time budgets. Extensive experiments show that ELECT significantly outperforms a wide range of basic UOMS baselines, including no model selection (always using the same popular model such as iForest) as well as more recent selection strategies based on meta-features.

==> tables/datasets.tex <==
\begin{table}[!htp]
\centering
	\caption{The wild testbed is composed by ODDS library (21 datasets) and DAMI library (18 datasets). The controlled testbed is created by injecting synthetic outliers into the datasets marked with *.} % title of Table
	\footnotesize
	\begin{tabular}{l l | r  r r } % centered columns (4 columns)
	\toprule
	 & \textbf{Data}                 & \textbf{Pts} & \textbf{Dim} & \textbf{\% Outlier} \\
	\midrule
    1 & annthyroid (ODDS)*             & 7200         & 6            & 7.4167                       \\
    2 & arrhythmia (ODDS)             & 452          & 274          & 14.6018                      \\
    3 & breastw (ODDS)*                & 683          & 9            & 34.9927                      \\
    4 & glass (ODDS)*                  & 214          & 9            & 4.2056                       \\
    5 & ionosphere (ODDS)*             & 351          & 33           & 35.8974                      \\
    6 & letter (ODDS)                 & 1600         & 32           & 6.25                         \\
    7 & lympho (ODDS)*                 & 148          & 18           & 4.0541                       \\
    8 & mammography (ODDS)*            & 11183        & 6            & 2.325                        \\
    9 & mnist (ODDS)                  & 7603         & 100          & 9.2069                       \\
    10 & musk (ODDS)                   & 3062         & 166          & 3.1679                       \\
    11 & optdigits (ODDS)              & 5216         & 64           & 2.8758                       \\
    12 & pendigits (ODDS)              & 6870         & 16           & 2.2707                       \\
    13 & pima (ODDS)*                   & 768          & 8            & 34.8958                      \\
    14 & satellite (ODDS)              & 6435         & 36           & 31.6395                      \\
    15 & satimage-2 (ODDS)             & 5803         & 36           & 1.2235                       \\
    % 16 & shuttle (ODDS)                & 49097        & 9            & 7.1511                       \\
    % 17 & smtp\_n (ODDS)                & 95156        & 3            & 0.0315                       \\
    16 & speech (ODDS)                 & 3686         & 400          & 1.6549                       \\
    17 & thyroid (ODDS)*                & 3772         & 6            & 2.4655                       \\
    18 & vertebral (ODDS)*              & 240          & 6            & 12.5                         \\
    19 & vowels (ODDS)                 & 1456         & 12           & 3.4341                       \\
    20 & wbc (ODDS)*                    & 378          & 30           & 5.5556                       \\
    21 & wine (ODDS)                   & 129          & 13           & 7.7519                       \\
    \midrule
    22 & ALOI (DAMI)                   & 49534        & 27           & 3.0444                       \\
    23 & Annthyroid (DAMI)             & 7129         & 21           & 7.4905                       \\
    24 & Arrhythmia (DAMI)             & 450          & 259          & 45.7778                      \\
    25 & Cardiotocography (DAMI)       & 2114         & 21           & 22.0435                      \\
    26 & Glass (DAMI)                  & 214          & 7            & 4.2056                       \\
    27 & HeartDisease (DAMI)           & 270          & 13           & 44.4444                      \\
    % 28 & Hepatitis (DAMI)              & 80           & 19           & 16.25                        \\
    28 & InternetAds (DAMI)            & 1966         & 1555         & 18.7182                      \\
    29 & PageBlocks (DAMI)             & 5393         & 10           & 9.4567                       \\
    30 & PenDigits (DAMI)              & 9868         & 16           & 0.2027                       \\
    31 & Pima (DAMI)                   & 768          & 8            & 34.8958                      \\
    32 & Shuttle (DAMI)                & 1013         & 9            & 1.2833                       \\
    33 & SpamBase (DAMI)               & 4207         & 57           & 39.9097                      \\
    34 & Stamps (DAMI)                 & 340          & 9            & 9.1176                       \\
    35 & Waveform (DAMI)               & 3443         & 21           & 2.9044                       \\
    36 & WBC (DAMI)                    & 223          & 9            & 4.4843                       \\
    37 & WDBC (DAMI)                   & 367          & 30           & 2.7248                       \\
    38 & Wilt (DAMI)                   & 4819         & 5            & 5.3331                       \\
    39 & WPBC (DAMI)                   & 198          & 33           & 23.7374                      \\
    \bottomrule
	\end{tabular}
	\label{table:datasets} % is used to refer this table in the text
\end{table}

==> tables/model_set.tex <==


\begin{table*}[!ht]
\footnotesize
\centering
\vspace{-0.1in}
	\caption{Outlier Detection Models; see hyperparameter definitions from PyOD } % title of Table
	\vspace{-0.15in}
	   \scalebox{0.9}{
	\begin{tabular}{lll|r} % centered columns (4 columns)
	    \toprule
		\textbf{Detection algorithm} &
		\textbf{Hyperparameter 1} & \textbf{Hyperparameter 2} & \textbf{Total}\\
		\midrule
		
		   LOF \citelatex{breunig2000lof}                             & n\_neighbors: $[1, 5 ,10, 15, 20, 25, 50, 60, 70, 80, 90, 100]$   & distance: ['manhattan', 'euclidean', 'minkowski'] & 36\\
		   
		    
		    kNN \citelatex{ramaswamy2000efficient}                      & n\_neighbors: $[1, 5 ,10, 15, 20, 25, 50, 60, 70, 80, 90, 100]$   & method: ['largest', 'mean', 'median'] & 36\\
		   
   
   		    OCSVM \citelatex{scholkopf2001estimating}                   & nu (train error tol): $[0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9]$    & kernel: ['linear', 'poly', 'rbf', 'sigmoid']  & 36\\
   
      
	COF \citelatex{tang2002enhancing}                           & n\_neighbors: $[3, 5, 10, 15, 20, 25, 50]$   & N/A & 7\\

		  ABOD \citelatex{kriegel2008angle}                           & n\_neighbors: $[3, 5, 10, 15, 20, 25, 50]$   & N/A  & 7\\

	
         iForest \citelatex{liu2008isolation}	    	         	& n\_estimators: $[10, 20, 30, 40, 50, 75, 100, 150, 200]$  & max\_features: $[0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9]$  & 81\\
   
         HBOS \citelatex{goldstein2012histogram}                     & n\_histograms: $[5, 10, 20, 30, 40, 50, 75, 100]$  & tolerance: $[0.1, 0.2, 0.3, 0.4, 0.5]$   & 40\\
   
   
       
		LODA \citelatex{pevny2016loda}                              & n\_bins: $[10, 20, 30, 40, 50, 75, 100, 150, 200]$        & n\_random\_cuts: $[5, 10, 15, 20, 25, 30]$ & 54\\
     
       
		\midrule
		&&& \textbf{297} \\ 
% 		\bottomrule
	\end{tabular}}
	\label{table:models_long} % is used to refer this table in the text
	\vspace{-0.3in}
\end{table*}





